Metrics for Evaluating Social Conformity of Crowd Navigation Algorithms

Recent protocols and metrics for training and evaluating autonomous robot navigation through crowds are inconsistent due to diversified definitions of "social behavior". This makes it difficult, if not impossible, to effectively compare published navigation algorithms. Furthermore, with the lack of a good evaluation protocol, resulting algorithms may fail to generalize, due to lack of diversity in training. To address these gaps, this paper facilitates a more comprehensive evaluation and objective comparison of crowd navigation algorithms by proposing a consistent set of metrics that accounts for both efficiency and social conformity, and a systematic protocol comprising multiple crowd navigation scenarios of varying complexity for evaluation. We tested four state-of-the-art algorithms under this protocol. Results revealed that some state-of-the-art algorithms have much challenge in generalizing, and using our protocol for training, we were able to improve the algorithm's performance. We demonstrate that the set of proposed metrics provides more insight and effectively differentiates the performance of these algorithms with respect to efficiency and social conformity.

==> Text/limitations.tex <==
We have evaluated the algorithms using simulation, like many existing works have done\cite{rgl,cadrlv2,sacadrl}, such that we can evaluate on a much large number of trials. In general to crowd navigation evaluation, it would be important to also evaluate in a real world setting, as there are sim-to-real gaps (especially between simulated and real human behaviors). However, this is more of a challenge to crowd navigation in general, and independent to our proposed metrics and protocol, as they can equally be used for evaluation in real world settings. In this paper, we have assumed that the robot is traveling by itself. Hence, we do not expect to have a human(s) that might be travelling closely along side the robot. If we are considering target applications where the robot is expected to travel closely beside a human(s) (e.g., a companion robot) , the scenarios in the proposed protocol and the metrics would need to be modified to account for this. For instance, $M_{I}$ should not penalize having the companion human(s) close to the robot. 

